Remplissage De L'Espace Euclidien Par Des Complexes Poly\'Edriques D'Orientation Impos\'Ee Et De Rotondit\'E Uniforme

We build polyhedral complexes in Rn that coincide with dyadic grids with different orientations, while keeping uniform lower bounds (depending only on n) on the flatness of the added polyhedrons including their subfaces in all dimensions. After the definitions and first properties of compact Euclidean polyhedrons and complexes, we introduce a tool allowing us to fill with n-dimensionnal polyhedrons a tubular-shaped open set, the boundary of which is a given n - 1-dimensionnal complex. The main result is proven inductively over n by completing our dyadic grids layer after layer, filling the tube surrounding each layer and using the result in the previous dimension to build the missing parts of the tube boundary. A possible application of this result is a way to find solutions to problems of measure minimization over certain topological classes of sets, in arbitrary dimension and codimension.

==> PolyedresABSTRACT.tex <==
\def\ABSTRACTonly{}
\input{Polyedres.tex}

